Thermodynamics and stability of non-equilibrium steady states in open systems

Thermodynamical arguments are known to be useful in the construction of physically motivated Lyapunov functionals for nonlinear stability analysis of spatially homogeneous equilibrium steady states in thermodynamically isolated systems. Unfortunately, the limitation to thermodynamically isolated systems is essential, and standard arguments are not applicable even for some very simple thermodynamically open systems. On the other hand, the nonlinear stability of thermodynamically open systems is usually investigated using the so-called energy method. Unfortunately, the designation "energy method" is clearly a misnomer. The mathematical quantity that is traditionally referred to as the "energy" is by no means linked to the energy in the physical sense of the word. Consequently, it would seem that genuine thermodynamical concepts are of no use in the nonlinear stability analysis of thermodynamically open systems. We show that this is not true. In particular, we propose a construction that in the case of simple heat conduction problem leads to a physically well-motivated Lyapunov functional, which effectively replaces the artificial Lyapunov functional used in the standard energy method. The proposed construction seems to be general enough to be applied in complex thermomechanical settings.

==> figures/plots/lyapunov-non-equilibrium-temperature-nonlinear-zoom.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(550,704){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(550,1518){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,2332){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,3147){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,3961){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,4775){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(682,484){\makebox(0,0){\strut{}$-\widehat{\vartemp}$}}%
      \csname LTb\endcsname%
      \put(3743,484){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%
      \put(2212,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(5273,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} }}%
      \put(176,2739){\makebox(0,0){\strut{}$g(\widetilde{\vartemp})$\ }}%
      \put(3742,154){\makebox(0,0){\strut{}$\widetilde{\vartemp}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}$a = 0.5$}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}$a = 0.2$}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}$a = 0.1$}}%
      \csname LTb\endcsname%
      \put(5816,3942){\makebox(0,0)[r]{\strut{}$a = 0.01$}}%
      \csname LTb\endcsname%
      \put(5816,3722){\makebox(0,0)[r]{\strut{}$a = 0.001$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{lyapunov-non-equilibrium-temperature-nonlinear-zoom}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/plots/lyapunov-non-equilibrium-temperature-nonlinear.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(550,704){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(550,1518){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,2332){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,3147){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,3961){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,4775){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(682,484){\makebox(0,0){\strut{}$-\widehat{\vartemp}$}}%
      \csname LTb\endcsname%
      \put(973,484){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%
      \put(2431,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(3888,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(5346,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} }}%
      \put(176,2739){\makebox(0,0){\strut{}$g(\widetilde{\vartemp})$\ }}%
      \put(3742,154){\makebox(0,0){\strut{}$\widetilde{\vartemp}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5816,3179){\makebox(0,0)[r]{\strut{}$a = 0.5$}}%
      \csname LTb\endcsname%
      \put(5816,2959){\makebox(0,0)[r]{\strut{}$a = 0.2$}}%
      \csname LTb\endcsname%
      \put(5816,2739){\makebox(0,0)[r]{\strut{}$a = 0.1$}}%
      \csname LTb\endcsname%
      \put(5816,2519){\makebox(0,0)[r]{\strut{}$a = 0.01$}}%
      \csname LTb\endcsname%
      \put(5816,2299){\makebox(0,0)[r]{\strut{}$a = 0.001$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{lyapunov-non-equilibrium-temperature-nonlinear}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/plots/lyapunov-non-equilibrium-temperature.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(550,704){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(550,1383){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,2061){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,2740){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,3418){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,4097){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,4775){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(682,484){\makebox(0,0){\strut{}$-\widehat{\temp}$}}%
      \csname LTb\endcsname%
      \put(1702,484){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%
      \put(2722,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(3743,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(4763,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(5783,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} }}%
      \put(176,2739){\makebox(0,0){\strut{}$g(\widetilde{\temp})$\ }}%
      \put(3742,154){\makebox(0,0){\strut{}$\widetilde{\temp}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3398,3987){\makebox(0,0)[r]{\strut{}$g(\widetilde{\temp}) = \frac{\widetilde{\temp}}{\widehat{\temp}} - \ln \left( 1 + \frac{\widetilde{\temp}}{\widehat{\temp}} \right)$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{lyapunov-non-equilibrium-temperature}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/plots/lyapunov-temperature.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(550,4775){\makebox(0,0)[r]{\strut{}0}}%
      \csname LTb\endcsname%
      \put(550,704){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,1383){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,2061){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,2740){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,3418){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(550,4097){\makebox(0,0)[r]{\strut{} }}%
      \csname LTb\endcsname%
      \put(682,484){\makebox(0,0){\strut{}0}}%
      \csname LTb\endcsname%
      \put(2212,484){\makebox(0,0){\strut{}$\temp=\temp_{\reference}$}}%
      \csname LTb\endcsname%
      \put(1447,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(2977,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(3743,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(4508,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(5273,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(6038,484){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{} }}%
      \put(176,2739){\makebox(0,0){\strut{}$f\left( \temp \right)$}}%
      \put(3742,154){\makebox(0,0){\strut{}$\temp$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5948,1273){\makebox(0,0)[r]{\strut{}$f\left( \temp \right) = \ln\left(\frac{\temp}{\temp_{\reference}}\right) + \frac{\temp}{\temp_{\reference}} -1$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{lyapunov-temperature}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/plots/stability-macros.tex <==
% Shifted net entropy functional
\newcommand{\entropyrellp}{{\mathcal S}}

% Shifted net total energy functional
\newcommand{\energyrellp}{{\mathcal E}}

% Relative entropy
\newcommand{\entropyrellpspec}{s_{\mathrm{rel}}}

% Temperature on the boundary
\newcommand{\tempbdr}{\temp_{\mathrm{bdr}}}

% Initial temperature
\newcommand{\tempinit}{\temp_{\mathrm{init}}}

% Energy in the standard energy method
\newcommand{\netstdenergy}{E_{\mathrm{std}}}

% Specific heat at constant volume, reference value
\newcommand{\cheatvolref}{\ensuremath{c_{\mathrm{V}, \reference}}}

% Temperature, different temperature scale
\newcommand{\vartemp}{\ensuremath{\vartheta}}

% Reference temperature
\newcommand{\tempref}{\ensuremath{\temp_{\reference}}}

% Reference temperature, different temperature scale
\newcommand{\vartempref}{\ensuremath{\vartemp_{\reference}}}

% Reference heat conductivity
\newcommand{\kapparef}{\ensuremath{\kappa_{\reference}}}


==> figures/plots/vit-prusa-macros-experimental.tex <==
%\makeatletter
% \@ifpackageloaded{tensor}% tensor is a package for a better typesetting of tensors
% {
% \renewcommand{\tnsr@Aux}[3][]{%
% \mathpalette{\tnsr@Plt{#1}{#3}}{\mathrm #2}%
% \tnsr@Wrn
% }%\tnsr@Aux
% }{%
% \relax%
% }
% \makeatother


% operators
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\Divergence}{Div}
\DeclareMathOperator{\gradient}{grad}
\DeclareMathOperator{\Gradient}{Grad}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\Asym}{Asym}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\signum}{sign}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\cof}{cof}

% jump
\newcommand{\jumpdis}[1]{\ensuremath{\left\lsem #1 \right\rsem}} % difference between function values at the point of jump discontinuity

% hyperbolic functions
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arccoth}{arccoth}

% invariants of second order tensor
\DeclareMathOperator{\invariantI}{I_1}
\DeclareMathOperator{\invariantII}{I_2}
\DeclareMathOperator{\invariantIII}{I_3}

% big o
\newcommand{\bigo}[1]{\ensuremath{O\left(#1 \right)}}
\newcommand{\smallo}[1]{\ensuremath{o\left(#1 \right)}}

% exponential
\newcommand{\exponential}[1]{\ensuremath{{\mathrm e}^{#1}}}

% imaginary unit
\newcommand{\iunit}{\ensuremath{\mathrm{i}}}


% real and imaginary part
\newcommand{\realp}{\mathrm{real}}
\newcommand{\imagp}{\mathrm{imag}}

%\newcommand{\Real}{\Re}
%\newcommand{\Imag}{\Im}
\providecommand{\Real}{\Re}
\providecommand{\Imag}{\Im}

% predicates
\newcommand{\charac}{\ensuremath{\mathrm{char}}} % characteristic quantity such as length scale, etc.
\newcommand{\reference}{\mathrm{ref}}
\newcommand{\crit}{\mathrm{crit}}
\newcommand{\bydefinition}{\mathrm{def}}
\newcommand{\traceless}[1]{{#1}_{\delta}}

% dimensionless variables and functions
\newcommand{\dimless}[1]{#1^\star}

% derivatives
\newcommand{\diff}{\mathrm{d}}
\newcommand{\Diff}[1][]{\mathrm{D}_{#1}} % For Frechet and Gateaux derivative

% inexact differential
\newcommand{\dbar}{{\mathchar'26\mkern-12mu \diff}}
\newcommand{\idiff}{\dbar}

% body
\newcommand{\body}{{\mathcal B}}

% vectors and tensors
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\greekvec}[1]{\ensuremath{\boldsymbol{#1}}}
\makeatletter
\@ifpackageloaded{bm}% 
{\renewcommand{\vec}[1]{\ensuremath{\bm{#1}}}%
\renewcommand{\greekvec}[1]{\ensuremath{\bm{#1}}}%
}{%
\relax% do nothing
}
\makeatother
\newcommand{\tensorq}[1]{\ensuremath{\mathbb{#1}}}      % tensorial quantity
\newcommand{\tensorc}[1]{\ensuremath{\mathrm{#1}}}      % tensorial quantity components  

\newcommand{\conjugate}[1]{#1^\star}
\newcommand{\transpose}[1]{#1^\top}
\newcommand{\transposei}[1]{#1^{-\top}}
\newcommand{\inverse}[1]{#1^{-1}}

% Identity matrix
\newcommand{\identity}{\ensuremath{\tensorq{I}}}

% Cauchy stress
\newcommand{\cstress}{\tensorq{T}}
\newcommand{\cstressc}{\tensorc{T}}

\newcommand{\ecstress}{\tensorq{S}}
\newcommand{\ecstressc}{\tensorc{S}}

% First Piola stress tensor
\newcommand{\fpstress}{\tensorq{T}_{\mathrm{R}}}
\newcommand{\fpstressc}{\tensorc{T}_{\mathrm R}}

% Second Piola--Kirchhoff stress tensor
\newcommand{\spstress}{\tensorq{S}_{\mathrm{R}}}
\newcommand{\spstressc}{\ensuremath{{{\mathrm S}_{\mathrm R}}}}

% Couple stress tensor
\newcommand{\couplestress}{\tensorq{M}}
\newcommand{\couplestressc}{\tensorc{M}}

% deformation, deformation gradient
\newcommand{\deformation}{\greekvec{\chi}}
\newcommand{\deformationc}{\tensorc{\chi}}

\newcommand{\fgrad}{\tensorq{F}}
\newcommand{\fgradc}{\tensorc{F}}
\newcommand{\fgradrel}[3][]{\fgrad^{#1}_{#2}\left(#3\right)}

% displacement
\newcommand{\displacement}{\vec{U}}
\newcommand{\displacementc}{\tensorc{U}}

% right Cauchy-Green tensor
\newcommand{\rcg}{\tensorq{C}}
\newcommand{\rcgc}{\tensorc{C}}        
\newcommand{\rcgrel}[3][]{\rcg^{#1}_{#2}\left(#3\right)}

% left Cauchy-Green tensor
\newcommand{\lcg}{\tensorq{B}}
\newcommand{\lcgc}{\tensorc{B}}        
\newcommand{\lcgrel}[3][]{\lcg^{#1}_{#2}\left(#3\right)}

%\newcommand{\piolastrain}{\tensorq{b}} % Piola deformation tensor (inverse of right Cauchy--Green)
%\newcommand{\fingerstrain}{\tensorq{c}} % Finger deformation tensor (inverse of left Cauchy--Green)

% rotation
\newcommand{\rotation}{\tensorq{R}}
\newcommand{\rotationrel}[3][]{\rotation^{#1}_{#2}\left(#3\right)}

% stretch
\newcommand{\stretchu}{\tensorq{U}}
\newcommand{\stretchurel}[3][]{\stretchu^{#1}_{#2}\left(#3\right)}
\newcommand{\stretchv}{\tensorq{V}}
\newcommand{\stretchvrel}[3][]{\stretchv^{#1}_{#2}\left(#3\right)}

% linearized strain (symmetric part of displacement gradient), skew-symmetric part of displacement gradient
\makeatletter
\@ifpackageloaded{bm}% 
{%
\newcommand{\linstrain}{\bbespilon} %requires \usepackage[bbgreekl]{mathbbol}
% YES, the spelling is wrong, but this is how it is coded in the package
}{%
\newcommand{\linstrain}{\tensorq{\varepsilon}}
}

\@ifpackageloaded{bm}%
{%
\newcommand{\skewdgradient}{\bbomega} 
}{%
\newcommand{\skewdgradient}{\tensorq{\omega}}
}

\@ifpackageloaded{bm}%
{%
\newcommand{\linstress}{\bbtau} % stress in linearise elasticity
}{%
\newcommand{\linstress}{\tensorq{\tau}}
}
\makeatother

\newcommand{\linstrainc}{\mathrm{\varepsilon}}
\newcommand{\linstressc}{\mathrm{\tau}}
\newcommand{\skewdgradientc}{\mathrm{\omega}}

% Lagrangean and Eulerian strain
\newcommand{\lstrain}{\tensorq{E}} % Green--Saint-Venant strain
\newcommand{\lstrainc}{\tensorc{E}} % Green--Saint-Venant strain, components
\newcommand{\estrain}{\tensorq{e}} % Euler--Almansi strain, components
\newcommand{\estrainc}{\tensorc{e}} % Euler--Almansi strain, components

% Rivlin-Ericksen tensor
\newcommand{\rivlin}{{\tensorq{A}}}

% generic tensor quantity
\newcommand{\generictensor}{{\tensorq{A}}}
\newcommand{\generictensorc}{\tensorc{A}} % component of the tensor

% deviatoric part of Cauchy stress
\newcommand{\dcstress}{\cstress - \left( \frac{1}{3}\Tr \cstress \right) \identity}
\newcommand{\dcstresssymb}{\traceless{\cstress}}

% mean normal stress
\newcommand{\cstressnorm}{\frac{1}{3}\Tr \cstress}

% velocity and velocity gradient, (skew)symmetric part of velocity gradient
\newcommand{\vecv}{\ensuremath{\vec{v}}}
\newcommand{\gradv}{\ensuremath{\nabla \vecv}}
\newcommand{\gradasym}{\ensuremath{\tensorq{W}}}
\newcommand{\gradsym}{\ensuremath{\tensorq{D}}}
\newcommand{\dgradsymsymb}{\ensuremath{\gradsym_{\delta}}}
\newcommand{\gradvl}{\ensuremath{\tensorq{L}}}

% surface velocity
\newcommand{\unders}[1]{\ensuremath{\underaccent{\mathrm{s}}{#1}}}

\newcommand{\gradsymop}{\nabla_{\mathrm{sym}}}
\newcommand{\gradasymop}{\nabla_{\mathrm{asym}}}

\newcommand{\vecvc}{\tensorc{v}}

% velocity and velocity gradient, (skew)symmetric part of velocity gradient, COMPONENTS
\newcommand{\gradsymc}{\tensorc{D}}
\newcommand{\gradasymc}{\tensorc{W}}

% functionals
\newcommand{\functional}[1]{{\mathfrak #1}}
\newcommand{\history}[3]{{\functional{#1}_{#2}^{#3}}}

% base vectors
\newcommand{\bvec}[1]{\vec{e}_{#1}} % current configuration
\newcommand{\Bvec}[1]{\vec{E}_{#1}} % reference configuration

% dual base vectors
\newcommand{\bvecd}[1]{\vec{e}^{#1}} % current configuration
\newcommand{\Bvecd}[1]{\vec{E}^{#1}} % reference configuration

% Cartesian basis, current configuration
\newcommand{\bvecx}{\bvec{\hat{x}}}
\newcommand{\bvecy}{\bvec{\hat{y}}}
\newcommand{\bvecz}{\bvec{\hat{z}}}

% Cartesian basis, reference configuration
\newcommand{\BvecX}{\Bvec{\hat{X}}}
\newcommand{\BvecY}{\Bvec{\hat{Y}}}
\newcommand{\BvecZ}{\Bvec{\hat{Z}}}

% Cartesian dual basis, reference configuration
\newcommand{\BvecdX}{\Bvecd{\hat{X}}}
\newcommand{\BvecdY}{\Bvecd{\hat{Y}}}
\newcommand{\BvecdZ}{\Bvecd{\hat{Z}}}

% Cartesian dual basis, current configuration
\newcommand{\bvecdx}{\bvecd{\hat{x}}}
\newcommand{\bvecdy}{\bvecd{\hat{y}}}
\newcommand{\bvecdz}{\bvecd{\hat{z}}}

% same as above but now in cylindrical coordinates
\newcommand{\bvecr}{\bvec{\hat{r}}}
\newcommand{\bvect}{\bvec{\hat{\theta}}}
\newcommand{\bvecp}{\bvec{\hat{\varphi}}}
%\newcommand{\bvecz}{\bvec{\hat{z}}}

\newcommand{\bvecdr}{\bvecd{\hat{r}}}
\newcommand{\bvecdt}{\bvecd{\hat{\theta}}}
\newcommand{\bvecdp}{\bvecd{\hat{\varphi}}}

\newcommand{\BvecR}{\Bvec{\hat{R}}}
\newcommand{\BvecP}{\Bvec{\hat{\Phi}}}
%\newcommand{\BvecZ}{\Bvec{\hat{Z}}}

\newcommand{\BvecdR}{\Bvecd{\hat{R}}}
\newcommand{\BvecdP}{\Bvecd{\hat{\Phi}}}
%\newcommand{\BvecdZ}{\Bvecd{\hat{Z}}}

% components
\newcommand{\vhatx}[1][\vecvc]{{#1}^{\hat{x}}}
\newcommand{\vhaty}[1][\vecvc]{{#1}^{\hat{y}}}
%\newcommand{\bvhatz}{\vhat{e}_{\hat{z}}}

\newcommand{\vhatr}[1][\vecvc]{{#1}^{\hat{r}}}
\newcommand{\vhatt}[1][\vecvc]{{#1}^{\hat{\theta}}}
\newcommand{\vhatp}[1][\vecvc]{{#1}^{\hat{\varphi}}}
\newcommand{\vhatz}[1][\vecvc]{{#1}^{\hat{z}}}

% indices
\newcommand{\hatx}{\hat{x}}
\newcommand{\haty}{\hat{y}}
\newcommand{\hatz}{\hat{z}}
\newcommand{\hatr}{\hat{r}}
\newcommand{\hatp}{\hat{\varphi}}
\newcommand{\hatt}{\hat{\theta}}
\newcommand{\hatX}{\hat{X}}
\newcommand{\hatY}{\hat{Y}}
\newcommand{\hatZ}{\hat{Z}}

% inner and outer radius (for some calcualtions)
\newcommand{\Rin}{R_{\mathrm{in}}}
\newcommand{\Rout}{R_{\mathrm{out}}}
\newcommand{\rin}{r_{\mathrm{in}}}
\newcommand{\rout}{r_{\mathrm{out}}}
 
% base vectors, abstract covariant and contravariant basis
\newcommand{\cobvec}[1]{\vec{g}_{#1}} % covariant base vector
\newcommand{\conbvec}[1]{\vec{g}^{#1}} % contravariant base vector
\newcommand{\cobvecn}[1]{\vec{g}_{\hat{#1}}} % covariant base vector
\newcommand{\conbvecn}[1]{\vec{g}^{\hat{#1}}} % contravariant base vector

\newcommand{\mtensor}{\tensorq{g}}  % metric tensor
\newcommand{\mtensorc}{{\mathrm g}} % metric tensor, components

% Christoffel symbols
\newcommand{\christoffel}[2]{\tensor{\Gamma}{^{#1}_{#2}}}

% mean curvature
\newcommand{\meancurvature}{\mathrm{K}} % mean curvature

\newcommand{\mtensorref}{\tensorq{G}}  %metric tensor in reference configuration
\newcommand{\mtensorrefc}{{\mathrm G}} %metric tensor in reference configuration, components

% Kronecker delta, Levi--Civitta symbol
\newcommand{\kdelta}[1]{\tensor{\delta}{#1}}
\newcommand{\lcepsilon}[1]{\tensor{\epsilon}{#1}}

% distributions
\newcommand{\diracdelta}{\delta}
\newcommand{\Heaviside}{H}

% hypergeometric function
\newcommand{\hypergeom}[4]{\ensuremath{ \mathrm{F}\left( \left[#1, #2 \right]; \left[ #3 \right]; #4\right)}}

% sets
\newcommand{\R}{\ensuremath{{\mathbb R}}}
\makeatletter
%\@ifpackageloaded{hyperref}% \C is defined in hyperref package
%{\renewcommand{\C}{\ensuremath{{\mathbb C}}}%
%}{%
%\newcommand{\C}{\ensuremath{{\mathbb C}}}%
%}
\makeatother
%\renewcommand{\C}{\ensuremath{{\mathbb C}}}% The lines above are no longer needed?
\newcommand{\Q}{\ensuremath{{\mathbb Q}}}
\newcommand{\N}{\ensuremath{{\mathbb N}}}
\newcommand{\Z}{\ensuremath{{\mathbb Z}}}


% Reynolds, Womersley number, etc.
\newcommand{\Reynolds}{\mathrm{Re}}
\newcommand{\Womersley}{\mathrm{Wo}}
\newcommand{\Rayleigh}{\mathrm{Ra}}
\newcommand{\RayleighSqrt}{\mathrm{R}}
\newcommand{\Prandtl}{\mathrm{Pr}}
\newcommand{\Grashof}{\mathrm{Gr}}
\newcommand{\Mach}{\mathrm{Ma}}
\newcommand{\Froude}{\mathrm{Fr}}
\newcommand{\Peclet}{\mathrm{Pe}}
\newcommand{\Eckert}{\mathrm{Ec}}
\newcommand{\Brinkman}{\mathrm{Br}}
\newcommand{\Nusselt}{\mathrm{Nu}}

% Young modulus, Poisson ratio
\newcommand{\Young}{\mathrm{E}}
\newcommand{\Poisson}{\mathrm{\nu}}

% Symetric and antisymetric tensors
\newcommand{\asym}[1]{\ensuremath{\Asym \left( #1 \right)}}
\newcommand{\sym}[1]{\ensuremath{\Sym \left( #1 \right)}}

% Energy, free energy, entropy, temperature
\newcommand{\tenergy}{\ensuremath{e}_{\mathrm{tot}}} % specific total energy (energy per unit mass), sum of specific internal energy and the specific kinetic energy
\newcommand{\ienergy}{\ensuremath{e}} % specific internal energy (energy per unit mass)
\newcommand{\menergy}{\ensuremath{e}_{\mathrm{mech}}} % specific mechanical energy (energy per unit mass), kinetic energy plus internal energy minus thermal contribution
\newcommand{\kenergy}{\ensuremath{e_{\mathrm{kin}}}} % specific kinetic energy (kinetic energy per unit mass)
\newcommand{\fenergy}{\ensuremath{\psi}} % specific free energy
\newcommand{\entropy}{\ensuremath{\eta}} % specific entropy
\newcommand{\entalphy}{\ensuremath{h}} % specific enthalpy
\newcommand{\gibbs}{\ensuremath{g}} % specific Gibbs free energy

\newcommand{\temp}{\ensuremath{\theta}} % temperature
\newcommand{\thpressure}{\ensuremath{p_{\mathrm{th}}}} % thermodynamic pressure
\newcommand{\mns}{\ensuremath{m}} % mean normal stress
\newcommand{\temptoref}{\ensuremath{\vartheta}} % (temperature - reference temperature)/(reference temperature)

% Net energy, free energy, entropy, ...
\newcommand{\nettenergy}{\ensuremath{E}_{\mathrm{tot}}} % net total energy
\newcommand{\netmenergy}{\ensuremath{E}_{\mathrm{mech}}} % net mechanical energy
\newcommand{\netthenergy}{\ensuremath{E}_{\mathrm{therm}}} % net thermal energy
\newcommand{\netienergy}{\ensuremath{E}} % net internal energy
\newcommand{\netkenergy}{\ensuremath{E_{\mathrm{kin}}}} % net kinetic energy
\newcommand{\netentropy}{\ensuremath{S}} % net entropy
\newcommand{\netheat}{\ensuremath{Q}} % net heat

% Specific molar gas constant
\newcommand{\Rspecific}{\ensuremath{R_{\mathrm{s}}}}
\newcommand{\Rmol}{\ensuremath{R_{\mathrm{m}}}}
 
% Specific heat at constant volume 
\newcommand{\cheatvol}{\ensuremath{c_{\mathrm{V}}}}

% Density in reference configuration
\newcommand{\rhor}{\rho_{\mathrm{R}}}

% Energy flux, heat flux, entropy flux
\newcommand{\efluxc}{\vec{j}_{e}} % energy flux, current configuration
\newcommand{\eflux}{\vec{J}_{e}} % energy flux, reference configuration

\newcommand{\hfluxc}{\vec{j}_{q}}     % heat flux, current configuration
\newcommand{\hfluxcc}{\tensorc{j}_{q}}     % heat flux, current configuration, components
\newcommand{\hflux}{\vec{J}_{q}}     % heat flux, reference configuration

\newcommand{\entfluxc}{\vec{j}_{\entropy}} % entropy flux, current configurtion 
\newcommand{\entflux}{\vec{J}_{\entropy}} % entropy flux, reference configuration

% Energy source, entropy source
\newcommand{\esourcec}{\ensuremath{q_{e}}} % energy source, current configuration
\newcommand{\hsourcec}{\ensuremath{q}} % heat source, current configuration
\newcommand{\entsourcec}{\ensuremath{q_{\entropy}}} % entropy source, current configuration

% Thermodynamical fluxes and affinities
\newcommand{\thfluxc}[1]{\vec{j}_{#1}} % thermodynamic flux, current configuration
\newcommand{\thaffinityc}[1]{\vec{a}_{#1}} % thermodynamic affinity, current configuration

% Entropy production
\newcommand{\entprodc}{\xi} % entorpy production, current configuration
\newcommand{\entprodctemp}{\zeta} % entorpy production times temperature, current configuration

% Derivatives, partial derivatives, covariant derivatives 
\newcommand{\pd}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\ppd}[2]{\ensuremath{\frac{\partial^2 {#1}}{\partial {#2^2}}}}
\newcommand{\dd}[2]{\ensuremath{\frac{\diff {#1}}{\diff {#2}}}}
\newcommand{\cd}[2]{\ensuremath{\frac{\diff^* {#1}}{\diff {#2}}}}
\newcommand{\ddd}[2]{\ensuremath{\frac{\diff^2 {#1}}{\diff {#2}^2}}}

% Upper convected (Oldroyd) derivative
\newcommand{\fid}[1]{\ensuremath{\accentset{\triangledown}{#1}}}
\newcommand{\fidd}[1]{\ensuremath{\accentset{\triangledown \! \triangledown}{#1}}}

% Lower convected derivative
\newcommand{\lfid}[1]{\ensuremath{\accentset{\meddiamond}{#1}}}
\newcommand{\lfidd}[1]{\ensuremath{\accentset{\meddiamond \! \meddiamond}{#1}}}

% Jaumann derivative
\newcommand{\jfid}[1]{\ensuremath{\accentset{\vartriangle}{#1}}}
\newcommand{\jfidd}[1]{\ensuremath{\accentset{\vartriangle \! \vartriangle}{#1}}}

% Green--Naghdi derivative
\newcommand{\gfid}[1]{\ensuremath{\accentset{\medsquare}{#1}}}
\newcommand{\gfidd}[1]{\ensuremath{\accentset{\medsquare \! \medsquare}{#1}}}

% Truesdell derivative
\newcommand{\tfid}[1]{\ensuremath{\accentset{\medcircle}{#1}}}
\newcommand{\tfidd}[1]{\ensuremath{\accentset{\medcircle \! \medcircle}{#1}}}

% Material derivative (\dot with \overline)
\newcommand{\mdif}[1]{\ensuremath{\dot{\overline{#1}}}}

\makeatletter
\@ifpackageloaded{tensor}% tensor is a package for a better typesetting of tensors
{
\newcommand{\codev}[2]{\ensuremath{\left. {#1} \right|\indices{_{#2}}}}
}{%
\newcommand{\codev}[2]{\ensuremath{\left. {#1} \right|_{#2}}}
}
\makeatother

\makeatletter
\@ifpackageloaded{tensor}% tensor is a package for a better typesetting of tensors
{
\newcommand{\contradev}[2]{\ensuremath{\left. {#1} \right|\indices{^{#2}}}}
}{%
\newcommand{\contradev}[2]{\ensuremath{\left. {#1} \right|^{#2}}}
}
\makeatother


% Bessel and Kelvin functions

\newcommand{\BesselI}[2]{\ensuremath{{\mathrm I}_{#1}\left(#2\right)}} 
\newcommand{\BesselK}[2]{\ensuremath{{\mathrm K}_{#1}\left(#2\right)}}
\newcommand{\BesselJ}[2]{\ensuremath{{\mathrm J}_{#1}\left(#2\right)}}
\newcommand{\BesselY}[2]{\ensuremath{{\mathrm Y}_{#1}\left(#2\right)}}

\newcommand\BesselRoot[2]{\ensuremath{{\rm j}_{#1,#2}}}

\newcommand{\KelvinBer}[2]{\ensuremath{{\mathrm{ber}}_{#1}\left(#2\right)}} 
\newcommand{\KelvinBei}[2]{\ensuremath{{\mathrm{bei}}_{#1}\left(#2\right)}}
\newcommand{\KelvinKer}[2]{\ensuremath{{\mathrm{ker}}_{#1}\left(#2\right)}}
\newcommand{\KelvinKei}[2]{\ensuremath{{\mathrm{kei}}_{#1}\left(#2\right)}}

% Chebyshev polynominals
\newcommand{\Chebyshevp}[3]{\ensuremath{{\mathrm T}_{#1}^{#2}\left(#3\right)}} 
\newcommand{\Chebyshev}[2]{\Chebyshevp{#1}{}{#2}} 

% norms
\newcommand{\norm}[2][]{\ensuremath{\left\|#2\right\|_{#1}}}
\newcommand{\absnorm}[1]{\ensuremath{\left|#1\right|}}

% volume
\makeatletter
\@ifundefined{volume}{%
\newcommand{\volume}[1][\Omega]{\ensuremath{#1}}}%
{%
\renewcommand{\volume}[1][\Omega]{\ensuremath{#1}}}
\makeatother

% surface and volume elements (reference configuration)
\newcommand{\svolume}[1][\Omega]{\ensuremath{\partial #1}}
\newcommand{\volumee}{\diff \mathrm{V}}
\newcommand{\surfacee}{\diff \vec{S}}
\newcommand{\surfacees}{\diff \mathrm{S}}
\newcommand{\linee}{\diff \vec{X}}

% surface and volume elements (current configuration)
\newcommand{\cvolumee}{\diff \mathrm{v}}
\newcommand{\csurfacee}{\diff \vec{s}}
\newcommand{\csurfacees}{\diff \mathrm{s}}
\newcommand{\clinee}{\diff \vec{x}}

% volume and surface integral
\newcommand{\intvolume}[2][\volume]{\int_{#1} #2\; \volumee}
\newcommand{\intsvolume}[2][\svolume]{\int_{#1} #2\; \surfacee}

% surface Jacobian
\newcommand{\surfacej}{\mathrm{j}}

% products
\newcommand{\tensortensor}[2]{\ensuremath{#1 \otimes #2}}
\makeatletter
\@ifpackageloaded{MnSymbol} % : as binary operator needs MnSymbol package
{
\newcommand{\tensordot}[2]{\ensuremath{#1 \vdotdot #2}} 
}{%
\newcommand{\tensordot}[2]{\ensuremath{#1 : #2}} 
}
\makeatother
\newcommand{\vectordot}[2]{\ensuremath{#1 \bullet #2}}
\newcommand{\vectorcross}[2]{\ensuremath{#1 \times #2}}

% function spaces
\newcommand{\scont}[2][\Omega]{\ensuremath{{\mathcal C}^{#2} \left(#1 \right)}}
\newcommand{\sdist}[1][\Omega]{\ensuremath{{\mathcal D} \left(#1 \right)}}
\newcommand{\sdistd}[1][\Omega]{\ensuremath{{\mathcal D}^\prime \left(#1 \right)}}

\newcommand{\scdiv}[1][\Omega]{\ensuremath{{\mathcal V} \left(#1 \right)}}

\newcommand{\loc}{\mathrm{loc}}

\newcommand{\slebl}[2]{\ensuremath{L}^{#1}_{\loc} \left(#2 \right)}
\newcommand{\sleb}[2]{\ensuremath{L}^{#1} \left(#2 \right)}


\newcommand{\ssob}[3]{\ensuremath{W}^{#1, #2} \left(#3 \right)}

% dualities, scalar products
\newcommand{\fadual}[4]{\left\langle #1, #2\right\rangle_{#3, #4}}
\newcommand{\fascal}[4]{\left\langle #1, #2\right\rangle_{#3, #4}}

% dual space
\newcommand{\dspace}[1]{#1^{\star}}

% tensorial function
\newcommand{\tensorf}[1]{{\mathfrak{#1}}}

% normal stress differences
\newcommand{\firstnsd}{N_1}
\newcommand{\secondnsd}{N_2}


==> figures/sketch/vit-prusa-macros-experimental.tex <==
%\makeatletter
% \@ifpackageloaded{tensor}% tensor is a package for a better typesetting of tensors
% {
% \renewcommand{\tnsr@Aux}[3][]{%
% \mathpalette{\tnsr@Plt{#1}{#3}}{\mathrm #2}%
% \tnsr@Wrn
% }%\tnsr@Aux
% }{%
% \relax%
% }
% \makeatother


% operators
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\Divergence}{Div}
\DeclareMathOperator{\gradient}{grad}
\DeclareMathOperator{\Gradient}{Grad}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\Asym}{Asym}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\signum}{sign}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\cof}{cof}

% jump
\newcommand{\jumpdis}[1]{\ensuremath{\left\lsem #1 \right\rsem}} % difference between function values at the point of jump discontinuity

% hyperbolic functions
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arccoth}{arccoth}

% invariants of second order tensor
\DeclareMathOperator{\invariantI}{I_1}
\DeclareMathOperator{\invariantII}{I_2}
\DeclareMathOperator{\invariantIII}{I_3}

% big o
\newcommand{\bigo}[1]{\ensuremath{O\left(#1 \right)}}
\newcommand{\smallo}[1]{\ensuremath{o\left(#1 \right)}}

% exponential
\newcommand{\exponential}[1]{\ensuremath{{\mathrm e}^{#1}}}

% imaginary unit
\newcommand{\iunit}{\ensuremath{\mathrm{i}}}


% real and imaginary part
\newcommand{\realp}{\mathrm{real}}
\newcommand{\imagp}{\mathrm{imag}}

%\newcommand{\Real}{\Re}
%\newcommand{\Imag}{\Im}
\providecommand{\Real}{\Re}
\providecommand{\Imag}{\Im}

% predicates
\newcommand{\charac}{\ensuremath{\mathrm{char}}} % characteristic quantity such as length scale, etc.
\newcommand{\reference}{\mathrm{ref}}
\newcommand{\crit}{\mathrm{crit}}
\newcommand{\bydefinition}{\mathrm{def}}
\newcommand{\traceless}[1]{{#1}_{\delta}}

% dimensionless variables and functions
\newcommand{\dimless}[1]{#1^\star}

% derivatives
\newcommand{\diff}{\mathrm{d}}
\newcommand{\Diff}[1][]{\mathrm{D}_{#1}} % For Frechet and Gateaux derivative

% inexact differential
\newcommand{\dbar}{{\mathchar'26\mkern-12mu \diff}}
\newcommand{\idiff}{\dbar}

% body
\newcommand{\body}{{\mathcal B}}

% vectors and tensors
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\greekvec}[1]{\ensuremath{\boldsymbol{#1}}}
\makeatletter
\@ifpackageloaded{bm}% 
{\renewcommand{\vec}[1]{\ensuremath{\bm{#1}}}%
\renewcommand{\greekvec}[1]{\ensuremath{\bm{#1}}}%
}{%
\relax% do nothing
}
\makeatother
\newcommand{\tensorq}[1]{\ensuremath{\mathbb{#1}}}      % tensorial quantity
\newcommand{\tensorc}[1]{\ensuremath{\mathrm{#1}}}      % tensorial quantity components  

\newcommand{\conjugate}[1]{#1^\star}
\newcommand{\transpose}[1]{#1^\top}
\newcommand{\transposei}[1]{#1^{-\top}}
\newcommand{\inverse}[1]{#1^{-1}}

% Identity matrix
\newcommand{\identity}{\ensuremath{\tensorq{I}}}

% Cauchy stress
\newcommand{\cstress}{\tensorq{T}}
\newcommand{\cstressc}{\tensorc{T}}

\newcommand{\ecstress}{\tensorq{S}}
\newcommand{\ecstressc}{\tensorc{S}}

% First Piola stress tensor
\newcommand{\fpstress}{\tensorq{T}_{\mathrm{R}}}
\newcommand{\fpstressc}{\tensorc{T}_{\mathrm R}}

% Second Piola--Kirchhoff stress tensor
\newcommand{\spstress}{\tensorq{S}_{\mathrm{R}}}
\newcommand{\spstressc}{\ensuremath{{{\mathrm S}_{\mathrm R}}}}

% Couple stress tensor
\newcommand{\couplestress}{\tensorq{M}}
\newcommand{\couplestressc}{\tensorc{M}}

% deformation, deformation gradient
\newcommand{\deformation}{\greekvec{\chi}}
\newcommand{\deformationc}{\tensorc{\chi}}

\newcommand{\fgrad}{\tensorq{F}}
\newcommand{\fgradc}{\tensorc{F}}
\newcommand{\fgradrel}[3][]{\fgrad^{#1}_{#2}\left(#3\right)}

% displacement
\newcommand{\displacement}{\vec{U}}
\newcommand{\displacementc}{\tensorc{U}}

% right Cauchy-Green tensor
\newcommand{\rcg}{\tensorq{C}}
\newcommand{\rcgc}{\tensorc{C}}        
\newcommand{\rcgrel}[3][]{\rcg^{#1}_{#2}\left(#3\right)}

% left Cauchy-Green tensor
\newcommand{\lcg}{\tensorq{B}}
\newcommand{\lcgc}{\tensorc{B}}        
\newcommand{\lcgrel}[3][]{\lcg^{#1}_{#2}\left(#3\right)}

%\newcommand{\piolastrain}{\tensorq{b}} % Piola deformation tensor (inverse of right Cauchy--Green)
%\newcommand{\fingerstrain}{\tensorq{c}} % Finger deformation tensor (inverse of left Cauchy--Green)

% rotation
\newcommand{\rotation}{\tensorq{R}}
\newcommand{\rotationrel}[3][]{\rotation^{#1}_{#2}\left(#3\right)}

% stretch
\newcommand{\stretchu}{\tensorq{U}}
\newcommand{\stretchurel}[3][]{\stretchu^{#1}_{#2}\left(#3\right)}
\newcommand{\stretchv}{\tensorq{V}}
\newcommand{\stretchvrel}[3][]{\stretchv^{#1}_{#2}\left(#3\right)}

% linearized strain (symmetric part of displacement gradient), skew-symmetric part of displacement gradient
\makeatletter
\@ifpackageloaded{bm}% 
{%
\newcommand{\linstrain}{\bbespilon} %requires \usepackage[bbgreekl]{mathbbol}
% YES, the spelling is wrong, but this is how it is coded in the package
}{%
\newcommand{\linstrain}{\tensorq{\varepsilon}}
}

\@ifpackageloaded{bm}%
{%
\newcommand{\skewdgradient}{\bbomega} 
}{%
\newcommand{\skewdgradient}{\tensorq{\omega}}
}

\@ifpackageloaded{bm}%
{%
\newcommand{\linstress}{\bbtau} % stress in linearise elasticity
}{%
\newcommand{\linstress}{\tensorq{\tau}}
}
\makeatother

\newcommand{\linstrainc}{\mathrm{\varepsilon}}
\newcommand{\linstressc}{\mathrm{\tau}}
\newcommand{\skewdgradientc}{\mathrm{\omega}}

% Lagrangean and Eulerian strain
\newcommand{\lstrain}{\tensorq{E}} % Green--Saint-Venant strain
\newcommand{\lstrainc}{\tensorc{E}} % Green--Saint-Venant strain, components
\newcommand{\estrain}{\tensorq{e}} % Euler--Almansi strain, components
\newcommand{\estrainc}{\tensorc{e}} % Euler--Almansi strain, components

% Rivlin-Ericksen tensor
\newcommand{\rivlin}{{\tensorq{A}}}

% generic tensor quantity
\newcommand{\generictensor}{{\tensorq{A}}}
\newcommand{\generictensorc}{\tensorc{A}} % component of the tensor

% deviatoric part of Cauchy stress
\newcommand{\dcstress}{\cstress - \left( \frac{1}{3}\Tr \cstress \right) \identity}
\newcommand{\dcstresssymb}{\traceless{\cstress}}

% mean normal stress
\newcommand{\cstressnorm}{\frac{1}{3}\Tr \cstress}

% velocity and velocity gradient, (skew)symmetric part of velocity gradient
\newcommand{\vecv}{\ensuremath{\vec{v}}}
\newcommand{\gradv}{\ensuremath{\nabla \vecv}}
\newcommand{\gradasym}{\ensuremath{\tensorq{W}}}
\newcommand{\gradsym}{\ensuremath{\tensorq{D}}}
\newcommand{\dgradsymsymb}{\ensuremath{\gradsym_{\delta}}}
\newcommand{\gradvl}{\ensuremath{\tensorq{L}}}

% surface velocity
\newcommand{\unders}[1]{\ensuremath{\underaccent{\mathrm{s}}{#1}}}

\newcommand{\gradsymop}{\nabla_{\mathrm{sym}}}
\newcommand{\gradasymop}{\nabla_{\mathrm{asym}}}

\newcommand{\vecvc}{\tensorc{v}}

% velocity and velocity gradient, (skew)symmetric part of velocity gradient, COMPONENTS
\newcommand{\gradsymc}{\tensorc{D}}
\newcommand{\gradasymc}{\tensorc{W}}

% functionals
\newcommand{\functional}[1]{{\mathfrak #1}}
\newcommand{\history}[3]{{\functional{#1}_{#2}^{#3}}}

% base vectors
\newcommand{\bvec}[1]{\vec{e}_{#1}} % current configuration
\newcommand{\Bvec}[1]{\vec{E}_{#1}} % reference configuration

% dual base vectors
\newcommand{\bvecd}[1]{\vec{e}^{#1}} % current configuration
\newcommand{\Bvecd}[1]{\vec{E}^{#1}} % reference configuration

% Cartesian basis, current configuration
\newcommand{\bvecx}{\bvec{\hat{x}}}
\newcommand{\bvecy}{\bvec{\hat{y}}}
\newcommand{\bvecz}{\bvec{\hat{z}}}

% Cartesian basis, reference configuration
\newcommand{\BvecX}{\Bvec{\hat{X}}}
\newcommand{\BvecY}{\Bvec{\hat{Y}}}
\newcommand{\BvecZ}{\Bvec{\hat{Z}}}

% Cartesian dual basis, reference configuration
\newcommand{\BvecdX}{\Bvecd{\hat{X}}}
\newcommand{\BvecdY}{\Bvecd{\hat{Y}}}
\newcommand{\BvecdZ}{\Bvecd{\hat{Z}}}

% Cartesian dual basis, current configuration
\newcommand{\bvecdx}{\bvecd{\hat{x}}}
\newcommand{\bvecdy}{\bvecd{\hat{y}}}
\newcommand{\bvecdz}{\bvecd{\hat{z}}}

% same as above but now in cylindrical coordinates
\newcommand{\bvecr}{\bvec{\hat{r}}}
\newcommand{\bvect}{\bvec{\hat{\theta}}}
\newcommand{\bvecp}{\bvec{\hat{\varphi}}}
%\newcommand{\bvecz}{\bvec{\hat{z}}}

\newcommand{\bvecdr}{\bvecd{\hat{r}}}
\newcommand{\bvecdt}{\bvecd{\hat{\theta}}}
\newcommand{\bvecdp}{\bvecd{\hat{\varphi}}}

\newcommand{\BvecR}{\Bvec{\hat{R}}}
\newcommand{\BvecP}{\Bvec{\hat{\Phi}}}
%\newcommand{\BvecZ}{\Bvec{\hat{Z}}}

\newcommand{\BvecdR}{\Bvecd{\hat{R}}}
\newcommand{\BvecdP}{\Bvecd{\hat{\Phi}}}
%\newcommand{\BvecdZ}{\Bvecd{\hat{Z}}}

% components
\newcommand{\vhatx}[1][\vecvc]{{#1}^{\hat{x}}}
\newcommand{\vhaty}[1][\vecvc]{{#1}^{\hat{y}}}
%\newcommand{\bvhatz}{\vhat{e}_{\hat{z}}}

\newcommand{\vhatr}[1][\vecvc]{{#1}^{\hat{r}}}
\newcommand{\vhatt}[1][\vecvc]{{#1}^{\hat{\theta}}}
\newcommand{\vhatp}[1][\vecvc]{{#1}^{\hat{\varphi}}}
\newcommand{\vhatz}[1][\vecvc]{{#1}^{\hat{z}}}

% indices
\newcommand{\hatx}{\hat{x}}
\newcommand{\haty}{\hat{y}}
\newcommand{\hatz}{\hat{z}}
\newcommand{\hatr}{\hat{r}}
\newcommand{\hatp}{\hat{\varphi}}
\newcommand{\hatt}{\hat{\theta}}
\newcommand{\hatX}{\hat{X}}
\newcommand{\hatY}{\hat{Y}}
\newcommand{\hatZ}{\hat{Z}}

% inner and outer radius (for some calcualtions)
\newcommand{\Rin}{R_{\mathrm{in}}}
\newcommand{\Rout}{R_{\mathrm{out}}}
\newcommand{\rin}{r_{\mathrm{in}}}
\newcommand{\rout}{r_{\mathrm{out}}}
 
% base vectors, abstract covariant and contravariant basis
\newcommand{\cobvec}[1]{\vec{g}_{#1}} % covariant base vector
\newcommand{\conbvec}[1]{\vec{g}^{#1}} % contravariant base vector
\newcommand{\cobvecn}[1]{\vec{g}_{\hat{#1}}} % covariant base vector
\newcommand{\conbvecn}[1]{\vec{g}^{\hat{#1}}} % contravariant base vector

\newcommand{\mtensor}{\tensorq{g}}  % metric tensor
\newcommand{\mtensorc}{{\mathrm g}} % metric tensor, components

% Christoffel symbols
\newcommand{\christoffel}[2]{\tensor{\Gamma}{^{#1}_{#2}}}

% mean curvature
\newcommand{\meancurvature}{\mathrm{K}} % mean curvature

\newcommand{\mtensorref}{\tensorq{G}}  %metric tensor in reference configuration
\newcommand{\mtensorrefc}{{\mathrm G}} %metric tensor in reference configuration, components

% Kronecker delta, Levi--Civitta symbol
\newcommand{\kdelta}[1]{\tensor{\delta}{#1}}
\newcommand{\lcepsilon}[1]{\tensor{\epsilon}{#1}}

% distributions
\newcommand{\diracdelta}{\delta}
\newcommand{\Heaviside}{H}

% hypergeometric function
\newcommand{\hypergeom}[4]{\ensuremath{ \mathrm{F}\left( \left[#1, #2 \right]; \left[ #3 \right]; #4\right)}}

% sets
\newcommand{\R}{\ensuremath{{\mathbb R}}}
\makeatletter
%\@ifpackageloaded{hyperref}% \C is defined in hyperref package
%{\renewcommand{\C}{\ensuremath{{\mathbb C}}}%
%}{%
%\newcommand{\C}{\ensuremath{{\mathbb C}}}%
%}
\makeatother
%\renewcommand{\C}{\ensuremath{{\mathbb C}}}% The lines above are no longer needed?
\newcommand{\Q}{\ensuremath{{\mathbb Q}}}
\newcommand{\N}{\ensuremath{{\mathbb N}}}
\newcommand{\Z}{\ensuremath{{\mathbb Z}}}


% Reynolds, Womersley number, etc.
\newcommand{\Reynolds}{\mathrm{Re}}
\newcommand{\Womersley}{\mathrm{Wo}}
\newcommand{\Rayleigh}{\mathrm{Ra}}
\newcommand{\RayleighSqrt}{\mathrm{R}}
\newcommand{\Prandtl}{\mathrm{Pr}}
\newcommand{\Grashof}{\mathrm{Gr}}
\newcommand{\Mach}{\mathrm{Ma}}
\newcommand{\Froude}{\mathrm{Fr}}
\newcommand{\Peclet}{\mathrm{Pe}}
\newcommand{\Eckert}{\mathrm{Ec}}
\newcommand{\Brinkman}{\mathrm{Br}}
\newcommand{\Nusselt}{\mathrm{Nu}}

% Young modulus, Poisson ratio
\newcommand{\Young}{\mathrm{E}}
\newcommand{\Poisson}{\mathrm{\nu}}

% Symetric and antisymetric tensors
\newcommand{\asym}[1]{\ensuremath{\Asym \left( #1 \right)}}
\newcommand{\sym}[1]{\ensuremath{\Sym \left( #1 \right)}}

% Energy, free energy, entropy, temperature
\newcommand{\tenergy}{\ensuremath{e}_{\mathrm{tot}}} % specific total energy (energy per unit mass), sum of specific internal energy and the specific kinetic energy
\newcommand{\ienergy}{\ensuremath{e}} % specific internal energy (energy per unit mass)
\newcommand{\menergy}{\ensuremath{e}_{\mathrm{mech}}} % specific mechanical energy (energy per unit mass), kinetic energy plus internal energy minus thermal contribution
\newcommand{\kenergy}{\ensuremath{e_{\mathrm{kin}}}} % specific kinetic energy (kinetic energy per unit mass)
\newcommand{\fenergy}{\ensuremath{\psi}} % specific free energy
\newcommand{\entropy}{\ensuremath{\eta}} % specific entropy
\newcommand{\entalphy}{\ensuremath{h}} % specific enthalpy
\newcommand{\gibbs}{\ensuremath{g}} % specific Gibbs free energy

\newcommand{\temp}{\ensuremath{\theta}} % temperature
\newcommand{\thpressure}{\ensuremath{p_{\mathrm{th}}}} % thermodynamic pressure
\newcommand{\mns}{\ensuremath{m}} % mean normal stress
\newcommand{\temptoref}{\ensuremath{\vartheta}} % (temperature - reference temperature)/(reference temperature)

% Net energy, free energy, entropy, ...
\newcommand{\nettenergy}{\ensuremath{E}_{\mathrm{tot}}} % net total energy
\newcommand{\netmenergy}{\ensuremath{E}_{\mathrm{mech}}} % net mechanical energy
\newcommand{\netthenergy}{\ensuremath{E}_{\mathrm{therm}}} % net thermal energy
\newcommand{\netienergy}{\ensuremath{E}} % net internal energy
\newcommand{\netkenergy}{\ensuremath{E_{\mathrm{kin}}}} % net kinetic energy
\newcommand{\netentropy}{\ensuremath{S}} % net entropy
\newcommand{\netheat}{\ensuremath{Q}} % net heat

% Specific molar gas constant
\newcommand{\Rspecific}{\ensuremath{R_{\mathrm{s}}}}
\newcommand{\Rmol}{\ensuremath{R_{\mathrm{m}}}}
 
% Specific heat at constant volume 
\newcommand{\cheatvol}{\ensuremath{c_{\mathrm{V}}}}

% Density in reference configuration
\newcommand{\rhor}{\rho_{\mathrm{R}}}

% Energy flux, heat flux, entropy flux
\newcommand{\efluxc}{\vec{j}_{e}} % energy flux, current configuration
\newcommand{\eflux}{\vec{J}_{e}} % energy flux, reference configuration

\newcommand{\hfluxc}{\vec{j}_{q}}     % heat flux, current configuration
\newcommand{\hfluxcc}{\tensorc{j}_{q}}     % heat flux, current configuration, components
\newcommand{\hflux}{\vec{J}_{q}}     % heat flux, reference configuration

\newcommand{\entfluxc}{\vec{j}_{\entropy}} % entropy flux, current configurtion 
\newcommand{\entflux}{\vec{J}_{\entropy}} % entropy flux, reference configuration

% Energy source, entropy source
\newcommand{\esourcec}{\ensuremath{q_{e}}} % energy source, current configuration
\newcommand{\hsourcec}{\ensuremath{q}} % heat source, current configuration
\newcommand{\entsourcec}{\ensuremath{q_{\entropy}}} % entropy source, current configuration

% Thermodynamical fluxes and affinities
\newcommand{\thfluxc}[1]{\vec{j}_{#1}} % thermodynamic flux, current configuration
\newcommand{\thaffinityc}[1]{\vec{a}_{#1}} % thermodynamic affinity, current configuration

% Entropy production
\newcommand{\entprodc}{\xi} % entorpy production, current configuration
\newcommand{\entprodctemp}{\zeta} % entorpy production times temperature, current configuration

% Derivatives, partial derivatives, covariant derivatives 
\newcommand{\pd}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\ppd}[2]{\ensuremath{\frac{\partial^2 {#1}}{\partial {#2^2}}}}
\newcommand{\dd}[2]{\ensuremath{\frac{\diff {#1}}{\diff {#2}}}}
\newcommand{\cd}[2]{\ensuremath{\frac{\diff^* {#1}}{\diff {#2}}}}
\newcommand{\ddd}[2]{\ensuremath{\frac{\diff^2 {#1}}{\diff {#2}^2}}}

% Upper convected (Oldroyd) derivative
\newcommand{\fid}[1]{\ensuremath{\accentset{\triangledown}{#1}}}
\newcommand{\fidd}[1]{\ensuremath{\accentset{\triangledown \! \triangledown}{#1}}}

% Lower convected derivative
\newcommand{\lfid}[1]{\ensuremath{\accentset{\meddiamond}{#1}}}
\newcommand{\lfidd}[1]{\ensuremath{\accentset{\meddiamond \! \meddiamond}{#1}}}

% Jaumann derivative
\newcommand{\jfid}[1]{\ensuremath{\accentset{\vartriangle}{#1}}}
\newcommand{\jfidd}[1]{\ensuremath{\accentset{\vartriangle \! \vartriangle}{#1}}}

% Green--Naghdi derivative
\newcommand{\gfid}[1]{\ensuremath{\accentset{\medsquare}{#1}}}
\newcommand{\gfidd}[1]{\ensuremath{\accentset{\medsquare \! \medsquare}{#1}}}

% Truesdell derivative
\newcommand{\tfid}[1]{\ensuremath{\accentset{\medcircle}{#1}}}
\newcommand{\tfidd}[1]{\ensuremath{\accentset{\medcircle \! \medcircle}{#1}}}

% Material derivative (\dot with \overline)
\newcommand{\mdif}[1]{\ensuremath{\dot{\overline{#1}}}}

\makeatletter
\@ifpackageloaded{tensor}% tensor is a package for a better typesetting of tensors
{
\newcommand{\codev}[2]{\ensuremath{\left. {#1} \right|\indices{_{#2}}}}
}{%
\newcommand{\codev}[2]{\ensuremath{\left. {#1} \right|_{#2}}}
}
\makeatother

\makeatletter
\@ifpackageloaded{tensor}% tensor is a package for a better typesetting of tensors
{
\newcommand{\contradev}[2]{\ensuremath{\left. {#1} \right|\indices{^{#2}}}}
}{%
\newcommand{\contradev}[2]{\ensuremath{\left. {#1} \right|^{#2}}}
}
\makeatother


% Bessel and Kelvin functions

\newcommand{\BesselI}[2]{\ensuremath{{\mathrm I}_{#1}\left(#2\right)}} 
\newcommand{\BesselK}[2]{\ensuremath{{\mathrm K}_{#1}\left(#2\right)}}
\newcommand{\BesselJ}[2]{\ensuremath{{\mathrm J}_{#1}\left(#2\right)}}
\newcommand{\BesselY}[2]{\ensuremath{{\mathrm Y}_{#1}\left(#2\right)}}

\newcommand\BesselRoot[2]{\ensuremath{{\rm j}_{#1,#2}}}

\newcommand{\KelvinBer}[2]{\ensuremath{{\mathrm{ber}}_{#1}\left(#2\right)}} 
\newcommand{\KelvinBei}[2]{\ensuremath{{\mathrm{bei}}_{#1}\left(#2\right)}}
\newcommand{\KelvinKer}[2]{\ensuremath{{\mathrm{ker}}_{#1}\left(#2\right)}}
\newcommand{\KelvinKei}[2]{\ensuremath{{\mathrm{kei}}_{#1}\left(#2\right)}}

% Chebyshev polynominals
\newcommand{\Chebyshevp}[3]{\ensuremath{{\mathrm T}_{#1}^{#2}\left(#3\right)}} 
\newcommand{\Chebyshev}[2]{\Chebyshevp{#1}{}{#2}} 

% norms
\newcommand{\norm}[2][]{\ensuremath{\left\|#2\right\|_{#1}}}
\newcommand{\absnorm}[1]{\ensuremath{\left|#1\right|}}

% volume
\makeatletter
\@ifundefined{volume}{%
\newcommand{\volume}[1][\Omega]{\ensuremath{#1}}}%
{%
\renewcommand{\volume}[1][\Omega]{\ensuremath{#1}}}
\makeatother

% surface and volume elements (reference configuration)
\newcommand{\svolume}[1][\Omega]{\ensuremath{\partial #1}}
\newcommand{\volumee}{\diff \mathrm{V}}
\newcommand{\surfacee}{\diff \vec{S}}
\newcommand{\surfacees}{\diff \mathrm{S}}
\newcommand{\linee}{\diff \vec{X}}

% surface and volume elements (current configuration)
\newcommand{\cvolumee}{\diff \mathrm{v}}
\newcommand{\csurfacee}{\diff \vec{s}}
\newcommand{\csurfacees}{\diff \mathrm{s}}
\newcommand{\clinee}{\diff \vec{x}}

% volume and surface integral
\newcommand{\intvolume}[2][\volume]{\int_{#1} #2\; \volumee}
\newcommand{\intsvolume}[2][\svolume]{\int_{#1} #2\; \surfacee}

% surface Jacobian
\newcommand{\surfacej}{\mathrm{j}}

% products
\newcommand{\tensortensor}[2]{\ensuremath{#1 \otimes #2}}
\makeatletter
\@ifpackageloaded{MnSymbol} % : as binary operator needs MnSymbol package
{
\newcommand{\tensordot}[2]{\ensuremath{#1 \vdotdot #2}} 
}{%
\newcommand{\tensordot}[2]{\ensuremath{#1 : #2}} 
}
\makeatother
\newcommand{\vectordot}[2]{\ensuremath{#1 \bullet #2}}
\newcommand{\vectorcross}[2]{\ensuremath{#1 \times #2}}

% function spaces
\newcommand{\scont}[2][\Omega]{\ensuremath{{\mathcal C}^{#2} \left(#1 \right)}}
\newcommand{\sdist}[1][\Omega]{\ensuremath{{\mathcal D} \left(#1 \right)}}
\newcommand{\sdistd}[1][\Omega]{\ensuremath{{\mathcal D}^\prime \left(#1 \right)}}

\newcommand{\scdiv}[1][\Omega]{\ensuremath{{\mathcal V} \left(#1 \right)}}

\newcommand{\loc}{\mathrm{loc}}

\newcommand{\slebl}[2]{\ensuremath{L}^{#1}_{\loc} \left(#2 \right)}
\newcommand{\sleb}[2]{\ensuremath{L}^{#1} \left(#2 \right)}


\newcommand{\ssob}[3]{\ensuremath{W}^{#1, #2} \left(#3 \right)}

% dualities, scalar products
\newcommand{\fadual}[4]{\left\langle #1, #2\right\rangle_{#3, #4}}
\newcommand{\fascal}[4]{\left\langle #1, #2\right\rangle_{#3, #4}}

% dual space
\newcommand{\dspace}[1]{#1^{\star}}

% tensorial function
\newcommand{\tensorf}[1]{{\mathfrak{#1}}}

% normal stress differences
\newcommand{\firstnsd}{N_1}
\newcommand{\secondnsd}{N_2}

